Decoding Social Sentiment in DAO: A Comparative Analysis of Blockchain Governance Communities

Blockchain technology is leading a revolutionary transformation across diverse industries, with effective governance being critical for the success and sustainability of blockchain projects. Community forums, pivotal in engaging decentralized autonomous organizations (DAOs), significantly impact blockchain governance decisions. Concurrently, Natural Language Processing (NLP), particularly sentiment analysis, provides powerful insights from textual data. While prior research has explored the potential of NLP tools in social media sentiment analysis, there is a gap in understanding the sentiment landscape of blockchain governance communities. The evolving discourse and sentiment dynamics on the forums of top DAOs remain largely unknown. This paper delves deep into the evolving discourse and sentiment dynamics on the public forums of leading DeFi projects: Aave, Uniswap, Curve DAO, Yearn.finance, Merit Circle, and Balancer, focusing primarily on discussions related to governance issues. Our study shows that participants in decentralized communities generally express positive sentiments during Discord discussions. Furthermore, there is a potential interaction between discussion intensity and sentiment dynamics; higher discussion volume may contribute to a more stable sentiment from code analysis. The insights gained from this study are valuable for decision-makers in blockchain governance, underscoring the pivotal role of sentiment analysis in interpreting community emotions and its evolving impact on the landscape of blockchain governance. This research significantly contributes to the interdisciplinary exploration of the intersection of blockchain and society, specifically emphasizing the decentralized blockchain governance ecosystem. We provide our data and code for replicability as open access on GitHub.

==> figs/data.tex <==
\begin{figure}[!htbp]
\centering
\includegraphics[width=\linewidth]{figs/data_processed_flowchart.pdf}
\caption{Data processed flowchart: created by Whimsical.}
\label{fig:data}
\end{figure}

==> figs/literature.tex <==
\begin{figure}[!htbp]
\centering
\includegraphics[width=\linewidth]{figs/literature-review-mandmap.pdf}
\caption{Literature review mindmap: created by Whimsical.}
\label{fig:literature}
\end{figure}

==> figs/whole.tex <==
\begin{figure}[!htbp]
\centering
\includegraphics[width=0.9\linewidth]{figs/whole_article_flowchart.pdf}
\caption{Overview of the article: created by Whimsical.}
\label{fig:overview}
\end{figure}

==> tabs/cite.tex <==
\begin{table*}[!htbp]
\centering
\caption{NLP Tools for Future Blockchain Governance Analysis}
\label{tab:nlp-tools}
\small % Reducing font size
\begin{tabular}{p{2cm}p{1cm} p{3.5cm}p{3.5cm}p{1.5cm} p{1cm}}
\toprule
\textbf{Name} & \textbf{Docs} & \multicolumn{2}{c}{\textbf{Application Scenarios}} & \textbf{Language} & \textbf{Open Access} \\
\cmidrule(lr){3-4}
& & \textbf{Social Media} & \textbf{Blockchain} & & \\ 
\midrule
\midrule

TextBlob & \href{https://textblob.readthedocs.io/en/dev/}{URL} & Diyasa, I. Gede Susrama Mas, et al. (2021) ~\cite{MasDiyasa_2021}& Hans, A., Mohadikar, K.R., Ekansh (2022) ~\cite{10.1007/978-981-16-8664-1_14} & Python & Yes: \href{https://github.com/sloria/textblob}{GitHub}\\

NLTK & \href{https://www.nltk.org/}{URL} & \href{https://www.iaeng.org/publication/IMECS2019/IMECS2019_pp12-16.pdf}{Elbagir, Shihab, Jing Yang (2019)} & Yang, Liuqing, et al. (2019)~\cite{10.1007/978-3-030-34083-4_13} & Python & Yes: \href{https://github.com/nltk/nltk}{GitHub} \\

Stanford CoreNLP & \href{https://stanfordnlp.github.io/CoreNLP/}{URL} & Kaur, Navjot, Arun Solanki (2018)~\cite{8442439} & \href{https://amset.umfst.ro/papers/2019-2/1_Cryptocurrency_DulauM_final_cu%20antet.pdf}{Dulău, Tudor-Mircea, Mircea Dulău (2019)} & Java & Yes: \href{https://github.com/stanfordnlp/CoreNLP}{GitHub} \\

spaCy & \href{https://spacy.io/usage/spacy-101}{URL} & Sharma, Mayank (2020) ~\cite{9197829} & Coulter, Kelly Ann (2022)~\cite{coulter2022impact} & Python & Yes: \href{https://github.com/explosion/spaCy}{GitHub} \\

FastText & \href{https://fasttext.cc/docs/en/support.html}{URL} & Raihan, Muhammad Afif, Erwin Budi Setiawan (2022)~\cite{MuhammadAfifRaihan_ErwinBudiSetiawan_2022} & Kilimci, Zeynep Hilal (2020)\cite{Kilimci_2020} & Python & Yes: \href{https://github.com/facebookresearch/fastText}{GitHub} \\

BERT & \href{https://arxiv.org/abs/1810.04805}{URL} & Heidari, Maryam, James H. Jones (2020)~\cite{9298158} & Ider, Duygu, Stefan Lessmann (2022)\cite{ider2023forecasting} & Python & Yes: \href{https://github.com/google-research/bert}{GitHub} \\

SentiWordNet & \href{https://github.com/aesuli/SentiWordNet/blob/master/papers/LREC10.pdf}{URL} & \href{https://ieeexplore.ieee.org/abstract/document/8843734}{Miranda, Eka, et al. (2019)}\cite{8843734} & \href{https://ethz.ch/content/dam/ethz/special-interest/mtec/chair-of-entrepreneurial-risks-dam/documents/dissertation/master%20thesis/Master%20Thesis%20Eisner_final.pdf}{Eisner, Lukas, Didier Sornette, Ke Wu (2019)} & N.A. & Yes: \href{https://github.com/aesuli/SentiWordNet}{GitHub} \\

Flair & \href{https://flairnlp.github.io/docs/intro}{URL} & \href{uqua.duke.edu/programs/mqm-business-analytics/admissions-facts-dates}{Kula, Sebastian, et al. (2020)} & McMillan, Benjamin, et al. (2022)\cite{AnalysisandComparison} & Python & Yes: \href{https://github.com/clips/pattern}{GitHub} \\

OpenAI-GPT & \href{https://platform.openai.com/docs/guides/gpt}{URL} & Wang, Zengzhi, et al.(2023) \cite{wang2023chatgpt}& N.A. & N.A. & No \\

\bottomrule

% Add more tools as needed
\end{tabular}
\end{table*}

